Improved early warning of compact binary mergers using higher modes of gravitational radiation: A population study

A gravitational-wave (GW) early-warning of a compact-binary coalescence event, with a sufficiently tight localisation skymap, would allow telescopes to point in the direction of the potential electromagnetic counterpart before its onset. This will enable astronomers to extract valuable information of the complex astrophysical phenomena triggered around the time of the merger. Use of higher-modes of gravitational radiation, in addition to the dominant mode typically used in templated real-time searches, was recently shown to produce significant improvements in early-warning times and skyarea localisations for a range of asymmetric-mass binaries. In this work, we perform a large-scale study to assess the benefits of this method for a population of compact binary merger observations. In particular, we inject 100,000 such signals in Gaussian noise, with component masses $m_1 \in \left[1, 60 \right] M_{\odot}$ and $m_2 \in \left [1, 3 \right] M_{\odot}$. We consider three scenarios involving ground-based detectors: the fifth (O5) observing run of the Advanced LIGO-Virgo-KAGRA network, its projected Voyager upgrade, as well as a proposed third generation (3G) network. We find that for fixed early warning times of $20-60$ seconds, the inclusion of the higher modes can provide localisation improvements of a factor of $\gtrsim 2$ for up to $\sim 60\%$ ($70 \%$) of the neutron star-black hole systems in the O5 (Voyager) scenario. Considering only those neutron star-black hole systems which can produce potential electromagnetic counterparts, such improvements in the localisation can be expected for $\sim 5-35\%$ $(20-50\%)$ binaries in O5 (Voyager), although the localisation areas themselves depend on the distances. For the 3G scenario, a significant fraction of the events have time gains of a minute to several minutes, assuming fiducial target localisation areas of 100 to 1000 sq. deg.

==> macros.tex <==
%%% General purpose macros
\newcommand{\ffrac}[2]{\ensuremath{\frac{\displaystyle #1}
                                        {\displaystyle #2}}}

\def\frmrtHz{\frac{\rm m}{\rtHz}}
\def\Msol{\ensuremath{\mathit{M_\odot}}}
\def\Msun{\Msol}
\def\Mcc{\Msol \ensuremath{\mathit{c}^2}}
\newcommand{\Mc}{\ensuremath{\mathcal{M}_c}}
\newcommand{\chieff}{\ensuremath{\chi_\mathrm{eff}}}

%%% New symbols and commands
\newcommand{\Ylm}{\ensuremath{Y_{\ell m}^{-2}(\iota, \varphi_{o})}}
\newcommand{\blambda}{\pmb{\lambda}}


%%% Various constants/measurements/units
\newcommand{\numevents}{56}
\newcommand{\sqdeg}{\ensuremath{\text{deg}^2}}

